CFVS: Coarse-to-Fine Visual Servoing for 6-DoF Object-Agnostic Peg-In-Hole Assembly

Robotic peg-in-hole assembly remains a challenging task due to its high accuracy demand. Previous work tends to simplify the problem by restricting the degree of freedom of the end-effector, or limiting the distance between the target and the initial pose position, which prevents them from being deployed in real-world manufacturing. Thus, we present a Coarse-to-Fine Visual Servoing (CFVS) peg-in-hole method, achieving 6-DoF end-effector motion control based on 3D visual feedback. CFVS can handle arbitrary tilt angles and large initial alignment errors through a fast pose estimation before refinement. Furthermore, by introducing a confidence map to ignore the irrelevant contour of objects, CFVS is robust against noise and can deal with various targets beyond training data. Extensive experiments show CFVS outperforms state-of-the-art methods and obtains 100%, 91%, and 82% average success rates in 3-DoF, 4-DoF, and 6-DoF peg-in-hole, respectively.

==> sections/03_1_coarse_approach.tex <==
% We present CFVS which consists of two components: (A) an open-loop control with the object-agnostic keypoint network (OAKN) and (B) a visual servoing with the offsets prediction network (OPN). The overall architecture is illustrated in Fig. \ref{fig:architecture}. For the OAKN and OPN, the input data is a 3D point cloud that is converted from a depth image captured by the eye-in-hand camera in the world coordinate. We use PointNet++ \cite{qi2017pointnet++} as a backbone network, which is widely adopted for 3D robotic manipulation.

We present CFVS, a coarse-to-fine 6-DoF peg-in-hole method comprised of two components: (A) the open-loop control with an object-agnostic keypoint network (OAKN) and (B) the visual servoing with an offsets prediction network (OPN), as shown in Fig.~\ref{fig:architecture}. 
%
% The input 3D point clouds that contain spatial information are reconstructed from depth images captured by the eye-in-hand camera in the world coordinate.
The input 3D point clouds are reconstructed from depth images captured by the eye-in-hand camera in the world coordinate, and then are sent to PointNet++~\cite{qi2017pointnet++}, a widely-adopted feature extractor for 3D robotic manipulation, to produce features for further processing.
%
% We then leverage PointNet++~\cite{qi2017pointnet++} as the feature extractor to comprehend the spatial relationship between the end-effector and target object, which is widely adopted for 3D robotic manipulation.


\subsection{Open-Loop Control with the Object-Agnostic Keypoint Network (OAKN)}
\label{sec:coarse}
%%%summary%%% 
%In the first stage, we move the end-effector, which is at a initial pose, to an bottleneck pose, which is close to a hole. For the reason that we just coarsely approach the hole in this stage, we design the OAKN to predict 3D hole keypoints, which are later converted to the approximate position and orientation of the hole. Then, the end-effector moves to that position and orientation.
%
To approximately reach the hole before refinement, we propose OAKN to predict the 3D keypoints around a hole, which will be used for position and orientation estimation.
%
% In the first stage, we move the end-effector from a initial pose to an bottleneck pose close to a hole. 
% %
% For the reason that we just coarsely approach the hole, we design the OAKN to predict 3D hole keypoints, which is later converted to the position and orientation of the hole. 
%

The OAKN extracts a 3D point cloud $X = \{x_i\}_{i=1}^{N} $ into the point features $\in \mathbb{R}^{N \times C}$ and predict three 3D hole keypoints. $N$ is the number of points and $x_i$ is in 3D coordinate. These 3D hole keypoints are calculated from the 3D keypoint offsets (Sec. \ref{sec:keypoint_offset}) and the confidence map that makes the framework object-agnostic (Sec. \ref{sec:heatmap}). Finally, the 3D hole keypoints are converted to the position and orientation of the hole and then the end-effector moves to that pose (Sec. \ref{sec:olc}). 

%In addition, the network is object-agnostic thanks to the confidence map which only focuses on the points near the center of the hole and ignores the contour of the object and whole scene.
\subsubsection{3D Keypoint Offsets}
\label{sec:keypoint_offset}
%%%summary%%%
% To estimate 3D hole keypoints, we first extract points into point features and then predict 3D keypoint offsets by each point. Given the position of each point, we add this position with 3D keypoint offsets to generate keypoint candidates. Then, combined with the confidence map that is described in the following section, we calculate the 3D hole keypoints.

The concept is similar to \cite{he2020pvn3d}. To estimate 3D hole keypoints, we first extract points into point features and then predict 3D keypoint offsets $\Delta K = \{\Delta k_{i,1},\Delta k_{i,2},\Delta k_{i,3}\}_{i=1}^{N} \in \mathbb{R}^{N \times 3}$ through several fully-connected layers. Then, we calculate the keypoint candidates $K = \{k_{i,1},k_{i,2},k_{i,3}\}_{i=1}^{N}$ from 3D keypoint offsets. The relationship between the keypoint candidates and the 3D keypoint offsets is defined as $k_{i,j} = x_i + \Delta k_{i,j}$, for all $i$ from $1$ to $N$ and $j$ from $1$ to $3$. Subsequently, we leverage keypoint candidates to calculate weighted average with confidence map (Sec.~\ref{sec:heatmap}) that is used as weights and obtain 3D hole keypoints for estimating the position and orientation of the hole (Sec.~\ref{sec:olc}).
% \forall 1 \leq i \leq N, 1 \leq j \leq 3$.
\subsubsection{Confidence Map}
\label{sec:heatmap}
%%%summary%%%
%To make the network object-agnostic, we introduce the confidence map, which is used to focus on the local points that are close to the hole and ignores the contour of the object and whole scene. We use the point features to predict the confidence map, which is later combined with keypoint candidates to generate 3D hole keypoints.

To make the network object-agnostic, we introduce the confidence map, which is used to focus on the local points that are close to the hole and ignores the contour of the object and whole scene. We feed point features into several fully-connected layers to predict the confidence map $\{w_i\}_{i=1}^{N} \in \mathbb{R}^{N \times 1}$, where $w_i$ is in the range $[0,1]$. We generate the ground-truth confidence map value $w_i^*$ from the 3D Gaussian function:
\begin{equation}
    w_i^* = e^{-\frac{1}{2\sigma^2}(\Vert x_i - p\Vert^2)},
\end{equation}

\noindent where $p$ is the position of hole center in 3D coordinate and $\sigma$ is used to control the range of the confidence map. If a point is closer to the position of the center, the value of confidence map will be larger. We refer to the confidence map as weights for calculating the 3D hole keypoints. Due to the confidence map, the network can be object-agnostic to predict more accurate 3D hole keypoints. 

\subsubsection{Open-Loop Control}
\label{sec:olc}
%%%summary%%%
% To approach the hole, we first estimate three 3D hole keypoints by calculating weighted average and then these keypoints are converted to the position and orientation of the hole. Then, we make the end-effector move to that pose.

To approach the hole, we first predict three 3D hole keypoints $\bar{K} = \{\bar{k}_1,\bar{k}_2,\bar{k}_3\}$ that is later converted to the position and orientation of the hole and $\bar{k}_1,\bar{k}_2,\bar{k}_3$ are in 3D coordinate. We obtain the 3D hole keypoints by calculating weighted average:
\begin{equation}
    \bar{k}_j = \frac{\sum^N_{i=1}k_{i,j} w_i}{\sum^N_{i=1}w_i},\ \forall j \in \{1,2,3\}.
\end{equation}

\noindent The first keypoint $\bar{k}_1$ is the center of hole and converted to translation $t \in \mathbb{R}^3$. The second $\bar{k}_2$ and third keypoint $\bar{k}_3$ is 25 mm greater than $\bar{k}_1$ along x-axis and z-axis, respectively, in the hole object frame. Thus, we can acquire the x-direction $v_x = \bar{k}_2 - \bar{k}_1$ and z-direction $v_z = \bar{k}_3 - \bar{k}_1$ of the hole pose. Next, we convert these two vectors to rotation matrix $R \in \mathbb{SO}^3$, as shown in Algorithm. \ref{alg:rot}. Then, we move the end-effector to the pose $[R|t] \in \mathbb{SE}^3$ through inverse kinematics. So far we have made the end-effector achieve the bottleneck pose that is needed to be adjusted by the following stage. (Sec. \ref{sec:fine})

\input{sections/algorithm/rotation_matrix}

\subsubsection{Loss} 
\label{sec:coarse_loss}
We train OAKN with supervised learning and the total loss is $L_{coarse} =  L_{kpts} +  L_{map}$, where $L_{kpts}$ and $L_{map}$ are the losses of 3D keypoint offsets and confidence map. We leverage the ground-truth 3D keypoint offsets $\{\Delta k^{*}_{i,1},\Delta k^{*}_{i,2},\Delta k^{*}_{i,3}\}_{i=1}^{N}$ and confidence map $\{w_i^*\}_{i=1}^{N}$ that is used as weights to reduce the influence of the shape of an object. Then, we adopt the weighted L1 loss to optimize the 3D keypoint offsets error:

\begin{equation}
        L_{kpts} = \frac{1}{N}\sum^N_{i=1}\sum^3_{j=1} w_i^* \Vert \Delta k_{i,j} - \Delta k^{*}_{i,j} \Vert.
\end{equation}
\noindent Subsequently, we use the root mean square error to minimize the confidence map error:

\begin{equation}
    L_{map} = \sqrt{\frac{1}{N}\sum^N_{i=1}\Vert h_i - h_i^* \Vert^2}.
\end{equation}





==> sections/tables/translation_error.tex <==
\begin{table}[htbp]
\caption{Alignment error of the successful case with 4mm clearance in 3-DoF peg-in-hole.}
\label{table:trans_err}
\begin{center}
%\centering
\setlength{\tabcolsep}{1mm}
\vspace{-6mm}
%\begin{tabular}{l|c|cccc}
\begin{tabular}{@{\extracolsep{2pt}}c||c|cccc@{}}

%
%\multicolumn{6}{c}{} \\
\hline
\multirow{3}{*}{Method} & \multirow{3}{*}{Avg.} & \multicolumn{2}{c}{Small shape variation} & \multicolumn{2}{c}{Large shape variation} \\
\cline{3-4} \cline{5-6} 
%\cmidrule(lr){3-4} \cmidrule(lr){5-6} 
& & \multirow{2}{*}{$\rm Cuboid_1$} & \multirow{2}{*}{$\rm Cuboid_2$} & \multirow{2}{*}{Cylinder} & Pentagonal \\
&&&&& prism \\
\hline
ICP w/ kpts \cite{besl1992method} & 0.0025 & 0.0018 & 0.0022 & 0.0020 & 0.0041  \\
3DRHD \cite{nigro2020peg} & 0.0016 & 0.0011 & 0.0013 & 0.0014 & 0.0026 \\
%\hline
KOVIS \cite{puang2020kovis} & 0.0039 & 0.0034 & 0.0024 & 0.0032 & 0.0066 \\
%\hline
CFVS (Ours) &  \textbf{0.0007} & \textbf{0.0006} & \textbf{0.0009} & \textbf{0.0005} & \textbf{0.0006} \\
\hline

\end{tabular}
\end{center}
\end{table}
